A Note on Linear Elliptic Systems on $\R^d$

We are concerned with the well-posedness of linear elliptic systems posed on $\mathbb{R}^d$. The concrete problem of interest, for which we require this theory, arises from the linearization of the equations of anisotropic finite elasticity, however, our results are more generally applicable to translation-invariant problem posed on $\mathbb{R}^d$. We describe a variant of homogeneous Sobolev spaces, which are convenient for treating problems of this kind.

==> notation.tex <==
% formatting in math environments
\renewcommand{\cases}[1]{\left\{ \begin{array}{rl} #1 \end{array} \right.}
\newcommand{\smfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\myvec}[1]{\left[ \begin{vector} #1 \end{vector} \right]}
\newcommand{\mymat}[1]{\left[ \begin{matrix} #1 \end{matrix} \right]}


% mean integral
\def\Xint#1{\mathchoice
{\XXint\displaystyle\textstyle{#1}}%
{\XXint\textstyle\scriptstyle{#1}}%
{\XXint\scriptstyle\scriptscriptstyle{#1}}%
{\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
\!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$ }
\vcenter{\hbox{$#2#3$ }}\kern-.6\wd0}}
% \def\ddashint{\Xint=}
\def\mint{\Xint-}


%% big, Big, bigg
\def\b{\big}
\def\B{\Big}
\def\bg{\bigg}
\def\Bg{\Bigg}

%% set separators
\def\sep{\,|\,}
\def\bsep{\,\b|\,}
\def\Bsep{\,\B|\,}

% Miscallaneous symbols
\def\diam{{\rm diam}}
\def\conv{{\rm conv}}
\def\t{\top} % matrix transpose (use $A^\transpose)
\def\argmin{{\rm argmin}}
\def\sign{{\rm sgn}}
\def\id{{\rm id}}

% fields
\def\R{\mathbb{R}}
\def\N{\mathbb{N}}
\def\Z{\mathbb{Z}}
\def\C{\mathbb{C}}

% spaces
\def\WW{W}
\def\CC{C}
\def\HH{H}
\def\LL{L}
\def\DD{\mathcal{D}'}

% integrals
\def\dx{\,{\rm d}x}
\def\dy{\,{\rm d}y}
\def\dz{\,{\rm d}z}
\def\dr{\,{\rm d}r}
\def\dt{\,{\rm d}t}
\def\ds{\,{\rm d}s}
\def\dd{{\rm d}}
\def\pp{\partial}
\def\dV{\,{\rm dV}}
\def\dA{\,{\rm dA}}
\def\db{\,{\rm db}}
\def\dlam{\,{\rm d}\lambda}
\def\dtheta{\,{\rm d}\theta}
\def\dk{\,{\rm d} k}

% duality pairing
\def\<{\langle}
\def\>{\rangle}

% shorcut for overline and underline
% overtilde, undertilde
\def\ol{\overline}
\def\ul{\underline}
\def\ot{\widetilde}
\newcommand{\ut}[1]{\underset{\widetilde{\hspace{2.5mm}}}{#1}}


% notation for matrices
\def\mA{{\sf A}}
\def\mB{{\sf B}}
\def\mF{{\sf F}}
\def\mG{{\sf G}}
\def\mH{{\sf H}}
\def\mI{{\sf I}}
\def\mJ{{\sf J}}
\def\mQ{{\sf Q}}
\def\mR{{\sf R}}
\def\mM{{\sf M}}
\def\mS{{\sf S}}

% notation for bold symbols
\def\bfa{{\bf a}}
\def\bfg{{\bf g}}


% \mathbb{...} notation (fourth-order tensors usually)
\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}





%% PAPER SPECIFIC DEFINITIONS

% Notation for derivatives:
\newcommand{\Da}[1]{D_{\!#1}}
\newcommand{\Dc}[1]{\partial_{#1}}
\def\D{\partial}
\def\del{\delta}
\def\ddel{\delta^2}
\def\dddel{\delta^3}

\def\DD{D}


% CO: just for me since it is difficult to type # on a Mac keyboard
% under emacs. will replace all occurances by \# though.
\def\per{\#}
\def\loc{{\rm loc}}

% atomic spacing
\def\eps{\varepsilon}
% shortcuts for sub and superscripts
\def\tot{{\rm tot}}
\def\cb{{\rm cb}}
\def\a{{\rm a}}
\def\c{{\rm c}}

% collection of notation
% \def\L{\mathscr{L}}
\def\L{{\Z^d}}
\def\Lper{\Z^d}
\def\Rg{\mathcal{R}}
\def\Ldir{\Z^d_*}

\def\Us{\mathscr{U}}
\def\Usper{\Us^\per}
\def\Usz{\Us^\per_0}
\def\Usc{\Us_{\rm c}}
\def\Ys{\mathscr{Y}}
\def\YsA{\mathscr{Y}_\mA}
\def\Yscdel{\Ys^\c_\delta}
\def\Ysdel{\Ys_\delta}
\def\Ysc{\Ys^\c}

\def\yF{y_\mF}
\def\yG{y_\mG}
\def\yB{y_\mB}
\def\yA{y_\mA}

\def\E{\mathscr{E}}
\def\Ea{\E^\a}
\def\Ec{\E^\c}
\def\Ech{\E^\c_h}



\def\Scb{\mS^\c}

\def\Pa{\mathscr{P}}
% \def\Pc{\mathscr{P}_\c}

\def\Eatot{\E_\a^\tot}
\def\Eatot{\E_\c^\tot}


\def\Om{{\R^d}}
\def\Omh{{\Omega_h}}
\def\Omc{\Omega^\c}
\def\Ombl{\Omega^\bl}

% 
\def\tily{\tilde y}
\def\tilz{\tilde z}
\def\tilu{\tilde u}
\def\tilv{\tilde v}
\def\tile{\tilde e}
\def\tilw{\tilde w}

\def\bary{\bar y}
\def\barz{\bar z}
\def\barv{\bar v}
\def\barw{\bar w}
\def\baru{\bar u}
\def\bare{\bar e}


% \def\ut{u^{\rm trig}}

% STRESS FUNCTIONS
\def\Sa{\mS^\a}
\def\Sc{\mS^\c}



\def\zz{\bar{\zeta}}
\def\zzid{\bar{\zeta}_{\rm 1D}}
\def\zzidper{\bar{\zeta}_{\rm 1D}^\per}
\def\zzper{\bar{\zeta}^\per}
\def\zzz{\tilde{\zeta}}
\def\zzzper{\tilde{\zeta}^\per}

\def\Sbar{\bar{\mathscr{S}}}
\def\Stil{\tilde{\mathscr{S}}}
\def\Sbarper{\bar{\mathscr{S}}^\per}
\def\Stilper{\tilde{\mathscr{S}}^\per}

\def\QQ{\mathscr{Q}}
\def\QQper{\QQ^\per}

\def\ww{\omega}
\def\DVdel{D^V_\mu}

% \def\Lama{\Lambda^\a}
\def\LamaN{\Lambda^\a}
\def\Lamc{\Lambda^\c}
\def\Lamainf{\Lambda^\a_\infty}
\def\Lamlh{\Lambda^{\rm LH}}

\def\Br{\mathcal{B}}
\def\BrN{\mathcal{B}_N}
\def\ii{\imath}
\def\Ha{\mathscr{H}_\a}
\def\Hc{\mathscr{H}_\c}

\def\Sta{\mathscr{S}^\a}
\def\Stc{\mathscr{S}^\c}

\def\tenC{{\bf C}}
